Screening of a test charge in a free-electron gas at warm dense matter and dense non-ideal plasma conditions

The screening of a test charge by partially degenerate non-ideal free electrons at conditions related to warm dense matter and dense plasmas is investigated using linear response theory and the local field correction based on ab inito Quantum Monte-Carlo simulations data. The analysis of the obtained results is performed by comparing to the random phase approximation and the Singwi-Tosi-Land-Sj\"olander approximation. The applicability of the long-wavelength approximation for the description of screening is investigated. The impact of electronic exchange-correlations effects on structural properties and the applicability of the screened potential from linear response theory for the simulation of the dynamics of ions are discussed.

==> old_bibitems.tex <==
\begin{thebibliography}{10}


\bibitem{quantum_theory} G.~Giuliani and G.~Vignale, Quantum Theory of the Electron Liquid, Cambridge University Press (2008)


\bibitem{loos} P.-F.~Loos and P.M.W.~Gill, The uniform electron gas, \href{http://onlinelibrary.wiley.com/doi/10.1002/wcms.1257/abstract}{ \textit{Comput.~Mol.~Sci.}~\textbf{6}, 410-429 } (2016)


\bibitem{review} T.~Dornheim, S.~Groth, and M.~Bonitz, The uniform electron gas at warm dense matter conditions,
\href{https://www.sciencedirect.com/science/article/abs/pii/S0370157318300516}{\textit{Phys.~Reports}~\textbf{744}, 1--86} (2018)

\bibitem{Dandrea_PRB}
R.G. Dandrea, N.W. Ashcroft, A.E. Carlsson, Electron liquid at any degeneracy, Phys. Rev. B {\bf 34}, 2097 (1986).




\bibitem{pines} D.~Bohm and D.~Pines, A Collective Description of Electron Interactions: II. Collective vs Individual Particle Aspects of the Interactions, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.85.338}{\textit{Phys.~Rev.}~\textbf{85}, 338} (1952)

\bibitem{bcs} J.~Bardeen, L.N.~Cooper, and J.R.~Schrieffer, Theory of superconductivity \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.108.1175}{\textit{Phys.~Rev.}~\textbf{108}, 1175} (1957)
















% Wigner crystallization

\bibitem{wigner} E.~Wigner, On the interaction of electrons in metals, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.46.1002}{\textit{Phys.~Rev.}~\textbf{46}, 1002} (1934)




\bibitem{drummond_wigner} N.D.~Drummond, Z.~Radnai, J.R.~Trail, M.D.~Towler, and R.J.~Needs, Diffusion quantum Monte Carlo study of three-dimensional Wigner crystals, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.69.085116}{\textit{Phys.~Rev.~B} \textbf{69}, 085116} (2004)









\bibitem{vwn} S.H.~Vosko, L.~Wilk, and M.~Nusair, Accurate Spin-Dependent Electron Liquid Correlation Energies for Local Spin Density Calculations: A Critical Analysis, \href{ http://www.nrcresearchpress.com/doi/abs/10.1139/p80-159}{ \textit{Can.~J.~Phys.}~\textbf{58}, 1200} (1980)


\bibitem{perdew} J.P.~Perdew and A.~Zunger, Self-interaction correction to density-functional approximations for many-electron systems, \href{ http://link.aps.org/doi/10.1103/PhysRevB.23.5048 }{ \textit{Phys.~Rev.~B} \textbf{23}, 5048 } (1981)

\bibitem{perdew_wang} J.P.~Perdew and Y.~Wang, Pair-distribution function and its coupling-constant average for the spin-polarized electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.46.12947}{\textit{Phys.~Rev.~B} \textbf{46}, 12947} (1992)

\bibitem{gori-giorgi1} P.~Gori-Giorgi, F.~Sacchetti, and G.B.~Bachelet, Analytic static structure factors and pair-correlation functions for the unpolarized homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.61.7353}{\textit{Phys.~Rev.~B} \textbf{61}, 7353} (2000)

\bibitem{gori-giorgi2} P.~Gori-Giorgi and J.P.~Perdew, Pair distribution function of the spin-polarized electron gas: A first-principles analytic model for all uniform densities, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.66.165118}{\textit{Phys.~Rev.~B} \textbf{66}, 165118} (2002)














\bibitem{gs2} D.M.~Ceperley and B.J.~Alder, Ground State of the Electron Gas by a Stochastic Method, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.45.566}{ \textit{Phys. Rev. Lett.} \textbf{45}, 566} (1980)





\bibitem{moroni2} S.~Moroni, D.M.~Ceperley, and G.~Senatore, Static Response and Local Field Factor of the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.75.689}{\textit{Phys.~Rev.~Lett.}~\textbf{75}, 689} (1995)


\bibitem{spink} G.G.~Spink, R.J.~Needs, and N.D.~Drummond, Quantum Monte Carlo study of the three-dimensional spin-polarized homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.88.085121}{\textit{Phys.~Rev.~B}~\textbf{88}, 085121} (2013)

\bibitem{ortiz1} G.~Ortiz and P.~Ballone, Correlation energy, structure factor, radial distribution function, and momentum distribution of the spin-polarized uniform electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.50.1391}{\textit{Phys.~Rev.~B} \textbf{50}, 1391} (1994)

\bibitem{ortiz2} G.~Ortiz, M.~Harris, and P.~Ballone, Zero Temperature Phases of the Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.82.5317}{\textit{Phys.~Rev.~Lett.}~\textbf{82}, 5317} (1999)








\bibitem{dft_review} R.O.~Jones, Density functional theory: Its origins, rise to prominence, and future, \href{ https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.87.897 }{ \textit{Rev.~Mod.~Phys.}~\textbf{87}, 897 } (2015)

\bibitem{burke_perspective} K.~Burke, Perspective on density functional theory, \href{https://aip.scitation.org/doi/10.1063/1.4704546}{\textit{J.~Chem.~Phys.}~\textbf{136}, 150901} (2012)




























% Giant planet interiors

\bibitem{militzer1} J.~Vorberger, I.~Tamblyn, B.~Militzer, and S.A.~Bonev, Hydrogen-helium mixtures in the interiors of giant planets, \href{ https://journals.aps.org/prb/abstract/10.1103/PhysRevB.75.024206 }{
\textit{Phys.~Rev.~B} \textbf{75}, 024206} (2007)



% ### Brown dwarfs
\bibitem{saumon1} D.~Saumon, W.B.~Hubbard, G.~Chabrier, and H.M.~van~Horn, The role of the
molecular-metallic transition of hydrogen in the evolution of Jupiter, Saturn, and
brown dwarfs, \href{http://adsabs.harvard.edu/full/1992ApJ...391..827S}{ \textit{Astrophys.~J.}~\textbf{391}, 827-831} (1992)


\bibitem{becker} A.~Becker, W.~Lorenzen, J.J.~Fortney, N.~Nettelmann, M.~Sch\"ottler, and R.~Redmer, Ab initio equations of state for
hydrogen (H-REOS.3) and helium (He-REOS.3) and their
implications for the interior of brown dwarfs, \href{https://iopscience.iop.org/article/10.1088/0067-0049/215/2/21/meta}{ \textit{Astrophys.~J.~Suppl.~Ser.}~\textbf{215}, 21} (2014)









% Fusion and stuff, ICF

\bibitem{hu_ICF} S.X.~Hu, B.~Militzer, V.N.~Goncharov, and S.~Skupsky, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.84.224109}{\textit{Phys.~Rev.~B} \textbf{84}, 224109} (2011)







\bibitem{torben_eur} T.~Ott, H.~Thomsen, J.W.~Abraham, T.~Dornheim, and M.~Bonitz, Recent progress in the theory and simulation of strongly correlated plasmas: phase transitions, transport, quantum, and magnetic field effects, \href{https://link.springer.com/article/10.1140/epjd/e2018-80385-7}{\textit{Eur.~Phys.~J.~D} \textbf{72}, 84} (2018)









% WDM experiment overview

\bibitem{falk_wdm} K.~Falk, Experimental methods for warm dense matter research, \href{https://www.cambridge.org/core/journals/high-power-laser-science-and-engineering/article/experimental-methods-for-warm-dense-matter-research/7205AE1029BEA0061044F84875F1CEDB}{\textit{High Power Laser Sci. Eng.}~\textbf{6}, e59} (2018)














% Spectacular experimental success:

\bibitem{exp1} D.~Kraus \textit{et al.}, Nanosecond formation of diamond and lonsdaleite by shock compression of graphite, \href{https://www.nature.com/articles/ncomms10970}{\textit{Nature Comm.}~\textbf{7}, 10970} (2016)

\bibitem{exp2} D.~Kraus \textit{et al.}, Formation  of  diamonds  in  laser-compressedhydrocarbons at planetary interior conditions, \href{https://www.nature.com/articles/s41550-017-0219-9?dom=prime&src=syn}{\textit{Nature Astronomy} \textbf{1}, 606-611} (2017)

\bibitem{exp3} A.L.~Kritcher, P.~Neumayer, J.~Castor, T.~D\"oppner, R.W.~Falcone, O.L.~Landen, H.J.~Lee, R.W.~Lee, E.C.~Morse, A.~Ng, S.~Pollaine, D.~Price, and S.H.~Glenzer, Ultrafast X-ray Thomson Scattering of Shock-Compressed Matter, \href{https://science.sciencemag.org/content/322/5898/69?casa_token=gnFVMXKwtFIAAAAA:-1mC8CHI-ffNXXfE2a6glDad_Von_3xGVRUUqpa8N6aOGGGsHxQvFletxgFvbnJLATqfGQHtB1LcWA}{\textit{Science} \textbf{322}, 69-71} (2008)

\bibitem{exp4}   M.Z.~Mo, Z.~Chen, R. K. Li, M. Dunning, B. B. L. Witte, J. K. Baldwin, L. B. Fletcher, J. B. Kim,A. Ng, R. Redmer, A. H. Reid, P. Shekhar, X. Z. Shen, M. Shen, K. Sokolowski-Tinten, Y. Y.Tsui, Y. Q. Wang, Q. Zheng, X. J. Wang, and S. H. Glenzer, Heterogeneous to homogeneous melting transition visualized with ultrafast electron diffraction, \href{https://science.sciencemag.org/content/360/6396/1451.abstract?casa_token=g9WE5wjZu_QAAAAA:WqzLgiMM_HQL3Yqil8pvJ0xu6EtKgDy61EpycMKXEJXbqxeAC1WTZeOlqDe4g0Cd2oyfb0jQtk9tag}{\textit{Science} \textbf{360}, 1451-1455} (2018)








% WDM theory general book

\bibitem{wdm_book} F.~Graziani, M.P.~Desjarlais, R.~Redmer, and S.B.~Trickey (eds.), Frontiers and Challenges in Warm Dense Matter, Springer International Publishing (2014)



\bibitem{new_POP} M.~Bonitz, T.~Dornheim, Zh.A.~Moldabekov, S.~Zhang, P.~Hamann, H.~K\"ahlert, A.~Filinov, K.~Ramakrishna, and J.~Vorberger, Ab initio simulation of warm dense matter,
\href{https://doi.org/10.1063/1.5143225}{\textit{Phys. Plasmas} \textbf{27} (4), 042710} (2020)


\bibitem{kas1} J.J.~Kas and J.J.~Rehr, Finite Temperature Green’s Function Approach for Excited State and Thermodynamic Properties of Cool to Warm Dense Matter, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.176403}{\textit{Phys.~Rev.~Lett.}~\textbf{119}, 176403} (2017)


\bibitem{kas3} T.S.~Tan, J.J.~Kas, and J.J.~Rehr, Coulomb-hole and screened exchange in the electron self-energy at finite temperature, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.98.115125}{\textit{Phys.~Rev.~B}~\textbf{98}, 115125} (2018)






% semi-classical MD

\bibitem{MD1} A.~Filinov, V.~Golubnychiy, M.~Bonitz, W.~Ebeling, and J.~Dufty, Temperature-dependent quantum pair potentials and their application to dense partially ionized hydrogen plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.70.046411}{\textit{Phys.~Rev.~E} \textbf{70}, 046411} (2004)

\bibitem{MD2} W.~Ebeling, A.~Filinov, M.~Bonitz, V.~Filinov, and T.~Pohl, 
The method of effective potentials in the quantum-statistical theory of plasmas, 
%Journal of Physics A: Mathematical and General
 \href{https://iopscience.iop.org/article/10.1088/0305-4470/39/17/S01/meta}{\textit{J.~Phys. A: Math.~Gen.}~\textbf{39}, 4309-4317} (2006)

















\bibitem{dornheim_sign_problem} T.~Dornheim, Fermion sign problem in path integral Monte Carlo simulations: Quantum dots, ultracold atoms, and warm dense matter, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.100.023307}{\textit{Phys.~Rev.~E} \textbf{100}, 023307} (2019)





\bibitem{loh} E.Y.~Loh, J.E.~Gubernatis, R.T.~Scalettar, S.R.~White, D.J.~Scalapino and R.L.~Sugar, Sign problem in the numerical simulation of many-electron systems, \href{http://link.aps.org/doi/10.1103/PhysRevB.41.9301}{\textit{Phys. Rev. B} \textbf{41}, 9301-9307} (1990)


\bibitem{troyer} M.~Troyer and U.J.~Wiese, Computational Complexity and Fundamental Limitations to Fermionic Quantum Monte Carlo Simulations, \href{http://link.aps.org/doi/10.1103/PhysRevLett.94.170201}{\textit{Phys. Rev. Lett.} \textbf{94}, 170201} (2005)













\bibitem{brown_ethan} E.W.~Brown, B.K.~Clark, J.L.~DuBois, and D.M.~Ceperley, Path-Integral Monte Carlo Simulation of the Warm Dense Homogeneous Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.110.146405}{\textit{Phys.~Rev.~Lett.}~\textbf{110}, 146405} (2013)







\bibitem{schoof_prl} T.~Schoof, S.~Groth, J.~Vorberger, and M.~Bonitz, \textit{Ab Initio} Thermodynamic Results for the Degenerate Electron Gas at Finite Temperature, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.115.130402}{\textit{Phys.~Rev.~Lett.}~\textbf{115}, 130402} (2015)






\bibitem{dornheim_prl} T.~Dornheim, S.~Groth, T.~Sjostrom, F.D.~Malone, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab Initio}   Quantum Monte Carlo Simulation of the Warm Dense Electron Gas in the Thermodynamic Limit, \href{ http://link.aps.org/doi/10.1103/PhysRevLett.117.156403}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 156403} (2016)



\bibitem{groth_prl} S.~Groth, T.~Dornheim, T.~Sjostrom, F.D.~Malone, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab initio} Exchange--Correlation Free Energy of the Uniform Electron Gas at Warm Dense Matter Conditions, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.119.135001}{\textit{Phys.~Rev.~Lett.}~\textbf{119}, 135001} (2017)




\bibitem{malone2} F.D.~Malone, N.S.~Blunt, E.W.~Brown, D.K.K.~Lee, J.S.~Spencer, W.M.C.~Foulkes, and J.J.~Shepherd, Accurate Exchange-Correlation Energies for the Warm Dense Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.117.115701}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 115701} (2016)

\bibitem{dornheim_pop} T.~Dornheim, S.~Groth, F.D.~Malone, T. Schoof, T.~Sjostrom, W.M.C.~Foulkes, and M.~Bonitz, \textit{Ab Initio}   Quantum Monte Carlo Simulation of the Warm Dense Electron Gas, \href{ http://aip.scitation.org/doi/full/10.1063/1.4977920}{ \textit{Phys.~Plasmas}  {\bf 24}, 056303} (2017)




















\bibitem{dornheim} T.~Dornheim, S.~Groth, A.~Filinov and M.~Bonitz, Permutation blocking path integral Monte Carlo: a highly efficient approach to the simulation of strongly degenerate non-ideal fermions, \href{ http://iopscience.iop.org/1367-2630/17/7/073017 }{ \textit{New J. Phys.} \textbf{17}, 073017} (2015)

\bibitem{dornheim2} T.~Dornheim, T.~Schoof, S.~Groth, A.~Filinov, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo Approach to the Uniform Electron Gas at Finite Temperature, \href{ http://scitation.aip.org/content/aip/journal/jcp/143/20/10.1063/1.4936145 }{ \textit{ J. Chem. Phys.} \textbf{143}, 204101} (2015)



\bibitem{groth} S.~Groth, T.~Schoof, T.~Dornheim, and M.~Bonitz, \textit{Ab Initio} Quantum Monte Carlo Simulations of the Uniform Electron Gas without Fixed Nodes, \href{ http://link.aps.org/doi/10.1103/PhysRevB.93.085102 }{ \textit{Phys.~Rev.~B} \textbf{93}, 085102} (2016)


\bibitem{dornheim3} T.~Dornheim, S.~Groth, T.~Schoof, C.~Hann, and M.~Bonitz, \textit{Ab initio} quantum Monte Carlo simulations of the Uniform electron gas without fixed nodes: The unpolarized case, \href{ http://link.aps.org/doi/10.1103/PhysRevB.93.205134 }{ \textit{Phys.~Rev.~B} \textbf{93}, 205134 } (2016)



\bibitem{dornheim_cpp} T.~Dornheim, S.~Groth, and M.~Bonitz, Ab initio results for the Static Structure Factor of the Warm Dense Electron Gas, \href{https://onlinelibrary.wiley.com/doi/full/10.1002/ctpp.201700096}{\textit{Contrib.~Plasma Phys.}~\textbf{57}, 468-478} (2017)



\bibitem{blunt} N.S.~Blunt, T.W.~Rogers, J.S.~Spencer, and W.M.C.~Foulkes, Density-matrix quantum Monte Carlo method, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.89.245124}{\textit{Phys.~Rev.~B} \textbf{89}, 245124} (2014)


\bibitem{malone1} F.D.~Malone, N.S.~Blunt, J.J.~Shepherd, D.K.K.~Lee, J.S.~Spencer, and W.M.C.~Foulkes, Interaction picture density matrix quantum Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.4927434}{\textit{J.~Chem.~Phys.}~\textbf{143}, 044116} (2015)

\bibitem{malone2} F.D.~Malone, N.S.~Blunt, E.W.~Brown, D.K.K.~Lee, J.S.~Spencer, W.M.C.~Foulkes, and J.J.~Shepherd, Accurate Exchange-Correlation Energies for the Warm Dense Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.117.115701}{\textit{Phys.~Rev.~Lett.}~\textbf{117}, 115701} (2016)




\bibitem{dornheim_neu} T.~Dornheim, S.~Groth, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo Simulations of Degenerate Electrons at Finite Temperature, \href{https://onlinelibrary.wiley.com/doi/full/10.1002/ctpp.201800157}{\textit{Contrib.~Plasma Phys.}~\textbf{59}, e201800157} (2019)














\bibitem{karasiev_status} V.V.~Karasiev, S.B.~Trickey, and J.W.~Dufty, Status of free-energy representations for the homogeneous electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.195134}{\textit{Phys.~Rev.~B} \textbf{99}, 195134} (2019)

















\bibitem{mermin_dft} N.D.~Mermin, Thermal Properties of the Inhomogeneous Electron Gas, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.137.A1441}{\textit{Phys.~Rev.}~\textbf{137}, A1441} (1965)

\bibitem{rajagopal_dft} U.~Gupta and A.K.~Rajagopal, Density functional formalism at finite temperatures with some applications, \href{https://www.sciencedirect.com/science/article/pii/0370157382900771}{\textit{Phys.~Reports} \textbf{87}, 259-311} (1982)





\bibitem{kushal} K.~Ramakrishna, T.~Dornheim, and J.~Vorberger, Influence of finite temperature Exchange-Correlation effects in Hydrogen, \href{https://arxiv.org/abs/2002.11574}{arxiv:2002.11574} (submitted for publication)





\bibitem{kugler1} A.A.~Kugler, Theory of the Local Field Correction in an Electron Gas, \href{ http://link.springer.com/article/10.1007/BF01024183}{ \textit{J.~Stat.~Phys.}~\textbf{12}, 35} (1975)















% advanced functionals for DFT

\bibitem{burke_ac} A.~Pribram-Jones, P.E.~Grabowski, and K.~Burke, Thermal Density Functional Theory: Time-Dependent Linear Response and Approximate Functionals from the Fluctuation-Dissipation Theorem, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.116.233001}{\textit{Phys.~Rev.~Lett.}~\textbf{116}, 233001} (2016)

\bibitem{lu_ac} D.~Lu, Evaluation of model exchange-correlation kernels in the adiabatic connection fluctuation-dissipation theorem for inhomogeneous systems, \href{https://aip.scitation.org/doi/10.1063/1.4867538}{\textit{J.~Chem.~Phys.}~\textbf{140}, 18A520} (2014)

\bibitem{patrick_ac} C.E.~Patrick and K.S.~Thygesen, Adiabatic-connection fluctuation-dissipation DFT for the structural properties of solids—The renormalized ALDA and electron gas kernels, \href{https://aip.scitation.org/doi/10.1063/1.4919236}{\textit{J.~Chem.~Phys.}~\textbf{143}, 102802} (2015)

\bibitem{goerling_ac} A.~G\"orling, Hierarchies of methods towards the exact Kohn-Sham correlation energy based on the adiabatic-connection fluctuation-dissipation theorem, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.235120}{\textit{Phys.~Rev.~B} \textbf{99}, 235120} (2019)






\bibitem{without_chihara} A.D.~Baczewski, L.~Shulenburger, M.P.~Desjarlais, S.B.~Hansen, and R.J.~Magyar, X-ray Thomson Scattering in Warm Dense Matter without the Chihara Decomposition, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.116.115004}{\textit{Phys.~Rev.~Lett.}~\textbf{116}, 115004} (2016)











\bibitem{diaw1} A.~Diaw and M.S.~Murillo, Generalized hydrodynamics model for strongly coupled plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.92.013107}{\textit{Phys.~Rev.~E} \textbf{92}, 013107} (2015)

\bibitem{diaw2} A.~Diaw and M.S.~Murillo, A viscous quantum hydrodynamics model based on dynamic density functional theory, \href{https://www.nature.com/articles/s41598-017-14414-9}{\textit{Sci.~Reports}~\textbf{7}, 15352} (2017)

\bibitem{zhanods_hydro} Zh.A.~Moldabekov, M.~Bonitz, and T.S.~Ramazanov, Theoretical foundations of quantum hydrodynamics for plasmas, \href{https://aip.scitation.org/doi/abs/10.1063/1.5003910}{\textit{Phys.~Plasmas} \textbf{25}, 031903} (2018)












\bibitem{ceperley_potential} G.~Senatore, S.~Moroni, and D.M.~Ceperley, Local field factor and effective potentials in liquid metals, \href{https://www.sciencedirect.com/science/article/pii/S002230939600316X}{\textit{J.~Non-Cryst.~Sol.}~\textbf{205-207}, 851-854} (1996)


\bibitem{zhandos1} Zh.A.~Moldabekov, S.~Groth, T.~Dornheim, H.~K\"ahlert, M.~Bonitz, and T.S.~Ramazanov, Structural characteristics of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.98.023207}{\textit{Phys.~Rev.~E} \textbf{98}, 023207} (2018)

\bibitem{zhandos2} Zh.A.~Moldabekov, H.~K\"ahlert, T.~Dornheim, S.~Groth, M.~Bonitz, and T.S.~Ramazanov, Dynamical structure factor of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.99.053203}{\textit{Phys.~Rev.~E} \textbf{99}, 053203} (2019)









\bibitem{siegfried_review} S.H.~Glenzer and R.~Redmer, X-ray Thomson scattering in high energy density plasmas, \href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.81.1625}{\textit{Rev.~Mod.~Phys.}~\textbf{81}, 1625} (2009)




\bibitem{kraus_xrts} D.~Kraus, B.~Bachmann, B.~Barbrel, R.W.~Falcone, L.B.~Fletcher, S.~Frydrych, E.J.~Gamboa, M.~Gauthier, D.O.~Gericke, S.H.~Glenzer, S.~G\"ode, E.~Granados, N.J.~Hartley, J.~Helfrich, H.J.~Lee, B.~Nagler, A.~Ravasio, W.~Schumaker, J.~Vorberger, and T.~D\"oppner, Characterizing the ionization potential depression in dense carbon plasmas with high-precision spectrally resolved x-ray scattering, \href{https://iopscience.iop.org/article/10.1088/1361-6587/aadd6c/meta}{\textit{Plasma Phys.~Control Fusion} \textbf{61}, 014015} (2019)






\bibitem{stopping2} D.O.~Gericke, M.~Schlanges, and W.D.~Kraeft, Stopping power of a quantum plasma---T-matrix approximation and dynamical screening, \href{https://www.sciencedirect.com/science/article/pii/0375960196006548}{\textit{Phys.~Lett.~A} \textbf{222}, 241-245} (1996)

\bibitem{stopping} Zh.A.~Moldabekov, T.~Dornheim, M.~Bonitz, and T.S.~Ramazanov, Ion energy loss characteristics and friction in a free electron gas at warm dense matter and non-ideal dense plasma conditions, 
\href{https://link.aps.org/doi/10.1103/PhysRevE.101.053203}{\textit{Phys. Rev. E} \textbf{101}, 053203} (2020)



\bibitem{Desjarlais:2017}
M.P.~Desjarlais, P.~Michael C.R.~Scullard, L.X.~Benedict, H.D.~Whitley, and R.~Redmer,
Density-functional calculations of transport properties in
the nondegenerate limit and the role of electron-electron scattering
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.95.033203}{\textit{Phys. Rev. E} \textbf{95}, 033203} (2017)


\bibitem{Veysman:2016} M.~Veysman, G.~R\"opke, M.~Winkel, and H.~Reinholz, Optical conductivity of warm dense matter within a wide
frequency range using quantum statistical and kinetic approaches
\href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.94.013203}{\textit{Phys. Rev. E},
  \textbf{94}, 013203} (2016)








\bibitem{jan_relax} J.~Vorberger, D.O.~Gericke, Th.~Bornath, and M.~Schlanges, Energy relaxation in dense, strongly coupled two-temperature plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.81.046404}{\textit{Phys.~Rev.~E} \textbf{81}, 046404} (2010)





\bibitem{moroni} S.~Moroni, D.M.~Ceperley, and G.~Senatore, 
Static response from quantum Monte Carlo calculations, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.69.1837}{\textit{Phys.~Rev.~Lett.}~\textbf{69}, 1837} (1992)









\bibitem{dynamic_folgepaper} S.~Groth, T.~Dornheim, and J.~Vorberger, \textit{Ab Initio} Path Integral Monte Carlo Approach to the Static and Dynamic Density Response of the Uniform Electron Gas, \href{https://link.aps.org/doi/10.1103/PhysRevB.99.235122}{\textit{Phys.~Rev.~B} \textbf{99}, 235122} (2019)



\bibitem{dornheim_ML} T.~Dornheim, J.~Vorberger, S.~Groth, N.~Hoffmann, Zh.A.~Moldabekov, and M.~Bonitz, The Static Local Field Correction of the Warm Dense Electron Gas: An ab Initio Path Integral Monte Carlo Study and Machine Learning Representation, \textit{J.~Chem.~Phys.}~(in press), \href{https://arxiv.org/abs/1907.08473}{arxiv:1907.08473}
























\bibitem{cdop} M.~Corradini, R.~Del Sole, G.~Onida, and M.~Palummo, Analytical Expressions for the Local-Field Factor $G(q)$ and the Exchange-Correlation Kernel ${K}_{\mathrm{xc}}(r)$ of the Homogeneous Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.57.14569}{ \textit{Phys.~Rev.~B} \textbf{57}, 14569} (1998)



% Parametrization of ground state properties





\bibitem{dornheim_EL} T.~Dornheim, T.~Sjostrom, S.~Tanaka, and J.~Vorberger, Strongly coupled electron liquid: Ab initio path integral Monte Carlo simulations and dielectric theories, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.101.045129}{\textit{Phys.~Rev.~B} \textbf{101}, 045129} (2020)

\bibitem{dornheim_HED} T.~Dornheim, Zh.A.~Moldabekov, J.~Vorberger, and S.~Groth, Ab initio path integral Monte Carlo simulation of the Uniform Electron Gas in the High Energy Density Regime, (Plasma Phys.~Control.~Fusion, in press)




\bibitem{dornheim_nonlinear} T.~Dornheim, J.~Vorberger, and M.~Bonitz, Nonlinear Electronic Density Response in Warm Dense Matter, \href{https://arxiv.org/abs/2004.03229}{arXiv:2004.03229} (submitted for publication)









\bibitem{dynamic_sign_problem} M.~Schiro, Real-time dynamics in quantum impurity models with diagrammatic Monte Carlo, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.81.085126}{\textit{Phys.~Rev.~B} \textbf{81}, 085126} (2010)

\bibitem{dynamic_sign_problem2} C.H.~Mak and R.~Egger, A multilevel blocking approach to the sign problem in real-time quantum Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.478077}{\textit{J.~Chem.~Phys.}~\textbf{110}, 12} (1999)






\bibitem{kwong} N.-H.~Kwong and M.~Bonitz, Real-Time Kadanoff-Baym Approach to Plasma Oscillations in a Correlated Electron Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.84.1768}{\textit{Phys.~Rev.~Lett.}~\textbf{84}, 1768} (2000)








\bibitem{takada1} Y.~Takada and H.~Yasuhara, Dynamical Structure Factor of the Homogeneous Electron Liquid: Its Accurate Shape and the Interpretation of Experiments on Aluminum, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.89.216402}{\textit{Phys.~Rev.~Lett.}~\textbf{89}, 216402} (2002)


\bibitem{takada2} Y.~Takada, Emergence of an excitonic collective mode in the dilute electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.94.245106}{\textit{Phys.~Rev.~B}~\textbf{94}, 245106} (2016)
































\bibitem{jarrell} M.~Jarrell and J.E.~Gubernatis, Bayesian inference and the analytic continuation of imaginary-time quantum Monte Carlo data, \href{https://www.sciencedirect.com/science/article/abs/pii/0370157395000747}{\textit{Phys.~Reports}~\textbf{269}, 133-195} (1996)


\bibitem{mem_revisited} Y.~Kora and M.~Boninsegni, Dynamic structure factor of superfluid $^4$He from quantum Monte Carlo: Maximum entropy revisited, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.98.134509}{\textit{Phys.~Rev.~B} \textbf{98}, 134509} (2018)

\bibitem{gift} E.~Vitali, M.~Rossi, and D.E.~Galli, \textit{Ab initio} low-energy dynamics of superfluid and solid $^4$He, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.82.174510}{\textit{Phys.~Rev.~B} \textbf{82}, 174510} (2010)

\bibitem{gift2} G.~Bertaina, D.E.~Galli, and E.~Vitali, Statistical and computational intelligence approach to analytic continuation in Quantum Monte Carlo, \href{https://www.tandfonline.com/doi/full/10.1080/23746149.2017.1288585}{\textit{Adv.~in Phys.: X} \textbf{2}, 302-329} (2017)

















\bibitem{dornheim_dynamic} T.~Dornheim, S.~Groth, J.~Vorberger, and M.~Bonitz, \textit{Ab initio} Path Integral Monte Carlo Results for the Dynamic Structure Factor of Correlated Electrons: From the Electron Liquid to Warm Dense Matter, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.121.255001}{\textit{Phys.~Rev.~Lett.}~\textbf{121}, 255001} (2018)














\bibitem{imada} M.~Takahashi and M.~Imada, Monte Carlo Calculation of Quantum Systems, \href{https://www.jstage.jst.go.jp/article/jpsj1946/53/3/53_3_963/_article/-char/ja/}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{53}, 963} (1984)

\bibitem{cep} D.M.~Ceperley, Path integrals in the theory of condensed helium, \href{http://link.aps.org/doi/10.1103/RevModPhys.67.279}{\textit{Rev. Mod. Phys.} \textbf{67}, 279-355} (1995)







\bibitem{trotter} H.~de Raedt and B.~de Raedt, Applications of the generalized Trotter formula, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.28.3575}{\textit{Phys.~Rev.~A} \textbf{28}, 3575} (1983)



\bibitem{HO1} L.~Brualla, K.~Sakkos, J.~Boronat, and J.~Casulleras, Higher order and infinite Trotter-number extrapolations in path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.1760512}{\textit{J.~Chem.~Phys.}~\textbf{121}, 636} (2004)

\bibitem{HO2} K.~Sakkos, J.~Casulleras, and J.~Boronat, High order Chin actions in path integral Monte Carlo, \href{https://aip.scitation.org/doi/full/10.1063/1.3143522}{\textit{J.~Chem.~Phys.}~\textbf{130}, 204109} (2009)










% Vanilla ground-state DFT review





\bibitem{groth_cpp} S.~Groth, T.~Dornheim, and M.~Bonitz, Free energy of the uniform electron gas: Testing analytical models against first‐principles results, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201600082}{\textit{Contrib.~Plasma Phys.}~\textbf{57}, 137-146} (2017)



















































































\bibitem{stls} S.~Tanaka and S.~Ichimaru, Thermodynamics and Correlational Properties of Finite-Temperature Electron Liquids in the Singwi-Tosi-Land-Sj\"olander Approximation, \href{ http://journals.jps.jp/doi/abs/10.1143/JPSJ.55.2278 }{ \textit{J.~Phys.~Soc.~Jpn.}~\textbf{55}, 2278-2289} (1986)


\bibitem{stls2} T.~Sjostrom, and J.~Dufty, Uniform Electron Gas at Finite Temperatures, \href{ http://link.aps.org/doi/10.1103/PhysRevB.88.115123 }{ \textit{Phys.~Rev.~B} \textbf{88}, 115123} (2013)



\bibitem{stls_original} K.S.~Singwi, M.P.~Tosi, R.H.~Land, and A.~Sj\"olander, Electron Correlations at Metallic Densities, \href{ http://link.aps.org/doi/10.1103/PhysRev.176.589}{ \textit{Phys.~Rev.}~\textbf{176}, 589} (1968)



\bibitem{vs_original} P.~Vashishta, and K.S.~Singwi, Electron Correlations at Metallic Densities. V, \href{ http://link.aps.org/doi/10.1103/PhysRevB.6.875}{ \textit{Phys.~Rev.~B} \textbf{6}, 875 } (1972)








\bibitem{tanaka_hnc} S.~Tanaka, Correlational and thermodynamic properties of finite-temperature electron liquids in the hypernetted-chain approximation, \href{https://aip.scitation.org/doi/abs/10.1063/1.4969071}{\textit{J.~Chem.~Phys.}~\textbf{145}, 214104} (2016)














\bibitem{dornheim_permutation_cycles} T.~Dornheim, S.~Groth, A.~Filinov, and M.~Bonitz, Path Integral Monte Carlo Simulation of Degenerate Electrons: Permutation-Cycle Properties, \href{https://aip.scitation.org/doi/10.1063/1.5093171}{\textit{J.~Chem.~Phys.}~\textbf{151}, 014108} (2019)













\bibitem{metropolis} N.~Metropolis, A.W.~Rosenbluth, M.N.~Rosenbluth, A.H.~Teller, and E.~Teller, Equation of State Calculations by Fast Computing Machines, \href{https://aip.scitation.org/doi/abs/10.1063/1.1699114}{\textit{J.~Chem.~Phys.}~\textbf{21}, 1087} (1953)
















\bibitem{velocity} E.~Rabani, D.R.~Reichman, G.~Krilov, and B.J.~Berne, The calculation of transport properties in quantum liquids using the maximum entropy numerical analytic continuation method: Application to liquid para-hydrogen, \href{https://www.pnas.org/content/99/3/1129}{\textit{PNAS} \textbf{99}, 1129-1133} (2002)



\bibitem{mezza} F.~Mezzacapo and M.~Boninsegni, Structure, superfluidity, and quantum melting of hydrogen clusters, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.75.033201}{\textit{Phys.~Rev.~A} \textbf{75}, 033201} (2007)





\bibitem{boninsegni1} M.~Boninsegni, N.V.~Prokofev, and B.V.~Svistunov, Worm algorithm and diagrammatic Monte Carlo: A new approach to continuous-space path integral Monte Carlo simulations, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.74.036701}{\textit{Phys.~Rev.~E}~\textbf{74}, 036701} (2006)

\bibitem{boninsegni2} M.~Boninsegni, N.V.~Prokofev, and B.V.~Svistunov, Worm Algorithm for Continuous-Space Path Integral Monte Carlo Simulations, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.96.070601}{\textit{Phys.~Rev.~Lett.}~\textbf{96}, 070601} (2006)












\bibitem{vanLeeuwen} G.~Stefanucci and R.~van Leeuwen, Nonequilibrium Many-Body Theory of Quantum Systems: A Modern Introduction, Cambridge University Press, Cambridge, United Kingdom, 2013







\bibitem{stls_1985} S.~Tanaka, S.~Mitake, and S.~Ichimaru, Parametrized equation of state for electron liquids in the Singwi-Tosi-Land-Sj\"olander approximation, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.32.1896}{\textit{Phys.~Rev.~A} \textbf{32}, 1896} (1985)









\bibitem{dynamic_i} T.~Hasegawa and M.~Shimizu, Electron correlations at metallic densities, II. Quantum mechanical expression of dielectric function with Wigner distribution function, \href{https://www.jstage.jst.go.jp/article/jpsj1946/38/4/38_4_965/_article/-char/ja/}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{38}, 965} (1975)




\bibitem{dynamic_iii} R.K.~Moudgil, P.K.~Ahluwalia, and K.N.~Pathak, Static and dynamic correlation functions of a two-dimensional quantum electron fluid, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.52.11945}{\textit{Phys.~Rev.~B} \textbf{52}, 11945} (1995)









\bibitem{arora} P.~Arora, K.~Kumar, and R.K.~Moudgil, Spin-resolved correlations in the warm-dense homogeneous electron gas, \href{https://link.springer.com/article/10.1140/epjb/e2017-70532-y}{\textit{Eur.~Phys.~J.~B}~\textbf{90}, 76} (2017)





\bibitem{stolzmann} W.~Stolzmann and M.~R\"osler, Static Local-Field Corrected Dielectric and Thermodynamic Functions, \href{ http://onlinelibrary.wiley.com/doi/10.1002/1521-3986(200103)41:2/3<203::AID-CTPP203>3.0.CO;2-S/abstract }{ \textit{Contrib.~Plasma Phys.}~\textbf{41}, 203} (2001)







\bibitem{lkw_fahrer} Zh.A.~Moldabekov, S.~Groth, T.~Dornheim, H.~K\"ahlert, M.~Bonitz, and T.S.~Ramazanov, Structural characteristics of strongly coupled ions in a dense quantum plasma, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.98.023207}{\textit{Phys.~Rev.~E} \textbf{98}, 023207} (2018)






\bibitem{bowen} G.~Sugiyama, C.~Bowen, and B.J.~Alder, Static dielectric response of charged bosons, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.46.13042}{\textit{Phys.~Rev.~B}~\textbf{46}, 13042} (1992)







\bibitem{bowen2} C.~Bowen, G.~Sugiyama, and B.J.~Alder, Static Dielectric Response of the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.50.14838}{\textit{Phys.~Rev.~B} \textbf{50}, 14838} (1994)










% Our primitive static response approach!


\bibitem{dornheim_pre} T.~Dornheim, S.~Groth, J.~Vorberger, and M.~Bonitz, Permutation Blocking Path Integral Monte Carlo approach to the Static Density Response of the Warm Dense Electron Gas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.96.023203}{\textit{Phys.~Rev.~E}~\textbf{96}, 023203} (2017)

\bibitem{groth_jcp} S.~Groth, T.~Dornheim, and M.~Bonitz, Configuration Path Integral Monte Carlo approach to the Static Density Response of the Warm Dense Electron Gas, \href{https://aip.scitation.org/doi/abs/10.1063/1.4999907}{\textit{J.~Chem.~Phys.}~\textbf{147}, 164108} (2017)











\bibitem{berne1} D.~Thirumalai and B.J.~Berne, On the calculation of time correlation functions in quantum systems: Path integral techniques, \href{https://aip.scitation.org/doi/abs/10.1063/1.445597}{\textit{J.~Chem.~Phys.}~\textbf{79}, 5029} (1983)


\bibitem{berne2} E.~Gallicchio and B.J.~Berne, The absorption spectrum of the solvated electron in fluid helium by maximum entropy inversion of imaginary time correlation functions from path integral Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.467892}{\textit{J.~Chem.~Phys.}~\textbf{101}, 9909} (1994)














\bibitem{fraser} L.M.~Fraser, W.M.C.~Foulkes, G.~Rajagopal, R.J.~Needs, S.D.~Kenny, and A.J.~Williamson, Finite-size effects and Coulomb interactions in quantum Monte Carlo calculations for homogeneous systems with periodic boundary conditions, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.53.1814}{\textit{Phys.~Rev.~B} \textbf{53}, 1814} (1996)


\bibitem{chiesa} S.~Chiesa, D.M.~Ceperley, R.M.~Martin, and M.~Holzmann, Finite-Size Error in Many-Body Simulations with Long-Range Interactions, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.97.076404}{\textit{Phys.~Rev.~Lett.}~\textbf{97}, 076404} (2006)

\bibitem{drummond} N.D.~Drummond, R.J.~Needs, A.~Sorouri, and W.M.C.~Foulkes, Finite-size errors in continuum quantum Monte Carlo calculations, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.78.125106}{\textit{Phys.~Rev.~B} \textbf{78}, 125106} (2008)


\bibitem{holzmann} M.~Holzmann, R.C.~Clay III, M.A.~Morales, N.M.~Tubman, D.M.~Ceperley, and C.~Pierleoni, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.94.035126}{\textit{Phys.~Rev.~B} \textbf{94}, 035126} (2016)













% ### Exciting new developments in the field of fermionic QMC simulations:




\bibitem{kugler_bounds} A.A.~Kugler, Bounds for Some Equilibrium Properties of an Electron Gas, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.1.1688}{\textit{Phys.~Rev.~A} \textbf{1}, 1688} (1970)






\bibitem{github_link} A link to a GitHub repository containing the PIMC data will be made available upon publication.









\bibitem{holas_limit} A.~Holas, Exact asymptotic expression for the static dielectric function of a uniform electron liquid at large wave vector,  in Strongly Coupled Plasma Physics, edited by F.J.~Rogers and H.E.~DeWitt (Plenum,NewYork,1987), p.46



\bibitem{negative_kxc_note} It is well known~\cite{neg1,neg2,stls} that $K_\text{xc}$ becomes negative for weak coupling above a certain temperature. Indeed, the negative large-$q$ asymptote of $G(q)$ predicted by Eq.~(\ref{eq:TAIL}) has recently been reported in this regime, see Ref.~\cite{dornheim_ML}.


\bibitem{neg1} B.~Militzer and E.L.~Pollock, Lowering of the Kinetic Energy in Interacting Quantum Systems, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.89.280401}{\textit{Phys.~Rev.~Lett.}~\textbf{89}, 280401} (2002)

\bibitem{neg2} W.D.~Kraeft, M.~Schlanges, J.~Vorberger, and H.E.~DeWitt, Kinetic and correlation energies and distribution functions of dense plasmas, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.66.046405}{\textit{Phys.~Rev.~E} \textbf{66}, 046405} (2002)




\bibitem{iyetomi_review} S.~Ichimaru, H.~Iyetomi, and S.~Tanaka, Statistical physics of dense plasmas: thermodynamics, transport coefficients and dynamic correlations, \href{https://www.sciencedirect.com/science/article/pii/0370157387901256}{\textit{Phys.~Reports} \textbf{149}, 91-205} (1987)







\bibitem{farid} B.~Farid, V.~Heine, G.E.~Engel, and I.J.~Robertson, Extremal Properties of the Harris-Foulkes Functional and an Improved Screening Calculation for the Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevB.48.11602}{\textit{Phys.~Rev.~B} \textbf{48}, 11602} (1993) 

\bibitem{kimball} J.C.~Kimball, Short-Range Correlations and Electron-Gas Response Functions, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.7.1648}{\textit{Phys.~Rev.~A} \textbf{7}, 1648} (1973)

\bibitem{bonitz_book} M. Bonitz, Quantum Kinetic Theory, 2nd ed. Springer 2016.

\bibitem{alexandrov_book} Alexandrov, Bogdankievich, Rukhadse, Plasma Electrodynamics











%\bibitem{feynman} R.P.~Feynman and A.R.~Hibbs, Quantum Mechanics and Path Integrals, Dover Publications, New York (2010)


%\bibitem{chandler} D.~Chandler and P.G.~Wolynes, Exploiting the isomorphism between quantum theory and classical statistical mechanics of polyatomic fluids, \href{https://aip.scitation.org/doi/abs/10.1063/1.441588}{\textit{J.~Chem.~Phys.}~\textbf{74}, 4078} (1981)


%\bibitem{kleinert} H.~Kleinert, Path Integrals in Quantum Mechanics, Statistics, Polymer Physics, and Financial Markets, World Scientific, Singapore, 2009









%\bibitem{curse} A.~Hinrichs, E.~Novak, M.~Ullrich and H.~Wozniakowski, The curse of dimensionality for numerical integration of smooth functions, \href{http://www.ams.org/journals/mcom/2014-83-290/S0025-5718-2014-02855-X/home.html}{\textit{Math.~Comp.}~\textbf{83}, 2853-2863} (2014)


%\bibitem{filinov_chapter} A.~Filinov and M.~Bonitz, Classical and Quantum Monte Carlo, \textit{Introduction to Computational Methods in Many Body Physic}, M.~Bonitz and D.~Semkat (Eds.), Rinton Press, Paramus (New Jersey) (2006)

%\bibitem{liu_monte_carlo} J.~Liu, Monte Carlo Strategies in Scientific Computing, Springer, New York (2013)


%\bibitem{pimc_original} L.D.~Fosdick and H.F.~Jordan, Path-Integral Calculation of the Two-Particle Slater Sum for He$^4$, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.143.58}{\textit{Phys.~Rev.}~\textbf{143}, 58} (1966)

%\bibitem{pimc_original2} H.F.~Jordan and L.D.~Fosdick, Three-Particle Effects in the Pair Distribution Function for He$^4$ Gas, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.171.128}{\textit{Phys.~Rev.}~\textbf{171}, 128} (1968)













% ### Crystal

%\bibitem{jones_crystal} M.D.~Jones and D.M.~Ceperley, Crystallization of the one-component plasma at finite temperature, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.76.4572}{\textit{Phys.~Rev.~Lett.}~\textbf{76}, 4572} (1996)


%\bibitem{filinov_PRL} A.V.~Filinov, M.~Bonitz, and Yu.E.~Lozovik, Wigner Crystallization in Mesoscopic 2D Electron Systems, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.86.3851}{\textit{Phys.~Rev.~Lett.}~\textbf{86}, 3851} (2001)













% ### Path Integral Monte Carlo (worm algorithm)


















%\bibitem{ceperley_fermions} D.M.~Ceperley, Path Integral Monte Carlo Methods for Fermions, \textit{Monte Carlo and Molecular Dynamics of Condensed Matter Systems}, K.~Binder and G.~Ciccotti (Eds.), Bologna (Italy) (1996)

























%\bibitem{wigner_molecule1} S.M.~Reimann, M.~Koskinen, and M.~Manninen, Formation of Wigner molecules in small quantum dots, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.62.8108}{\textit{Phys.~Rev.~B}~\textbf{62}, 8108} (2000)

%\bibitem{wigner_molecule2} B.~Reusch, W.~H\"ausler, and H.~Grabert, Wigner molecules in quantum dots, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.63.113313}{\textit{Phys.~Rev.~B}~\textbf{63}, 113313} (2001)

%\bibitem{wigner_molecule3} E.~R\"as\"anen, H.~Saarikoski, M.J.~Puska, and R.M.~Nieminen, Wigner molecules in polygonal quantum dots: A density-functional study, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.67.035326}{\textit{Phys.~Rev.~B}~\textbf{87}, 035326} (2003)




%\bibitem{ross} M.~Ross, Matter under extreme conditions of temperature and pressure, \href{https://doi.org/10.1088\%2F0034-4885\%2F48\%2F1\%2F001}{\textit{Rep.~Prog.~Phys.}~\textbf{48}, 1--52} (1985)

%\bibitem{koenig} M.~Koenig \textit{et al.}, Progress in the study of warm dense matter, \href{https://doi.org/10.1088\%2F0741-3335\%2F47\%2F12b\%2Fs31}{\textit{Plasma Phys.~Control.~Fusion} \textbf{47}, B441--B449} (2005)



%\bibitem{fortov_review} V.E.~Fortov, Extreme states of matter on Earth and in space, \href{https://www.turpion.org/php/paper.phtml?journal_id=pu&paper_id=6821}{\textit{Phys.-Usp.}~\textbf{52}, 615--647} (2009)















%\bibitem{brown_chapter} E.~Brown, M.A.~Morales, C.~Pierleoni, and D.~Ceperley, Quantum Monte Carlo Techniques and Applications for Warm Dense
%Matter, in F. Graziani, M. P. Desjarlais, R. Redmer, and S. B.
%Trickey (Eds.), \textit{Frontiers and Challenges in Warm Dense Matter},
%Springer International Publishing (2014)



































%\bibitem{brenda} Y.~Liu, M.~Cho, and B.~Rubenstein, \textit{Ab Initio} Finite Temperature Auxiliary Field Quantum Monte Carlo, \href{https://pubs.acs.org/doi/abs/10.1021/acs.jctc.8b00569}{\textit{J.~Chem.~Theory~Comput.}~\textbf{14}, 4722-4732} (2018)


%\bibitem{universe} V.~Filinov and A.~Larkin, Quantum Dynamics of Charged Fermions in the Wigner Formulation of Quantum Mechanics, \href{https://www.mdpi.com/2218-1997/4/12/133/htm}{\textit{Universe} \textbf{4}, 133} (2018)












%\bibitem{trotter} H.~De Raedt and B.~De Raedt, Applications of the generalized Trotter formula, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.28.3575}{\textit{Phys.~Rev.~A} \textbf{28}, 3575} (1983)






%\bibitem{fermion_nodes} D.M.~Ceperley, Fermion nodes, \href{https://link.springer.com/article/10.1007/BF01030009}{\textit{J.~Stat.~Phys.}~\textbf{63}, 1237-1267} (1991)









%\bibitem{dornheim_analyzing} T.~Dornheim, H.~Thomsen, P.~Ludwig, A.~Filinov, and M.~Bonitz, Analyzing Quantum Correlations Made Simple, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201500120}{\textit{Contrib.~Plasma Phys.}~\textbf{56}, 371-379} (2016)






%\bibitem{reimann} S.M.~Reimann and M.~Manninen, Electronic structure of quantum dots, \href{https://journals.aps.org/rmp/abstract/10.1103/RevModPhys.74.1283}{\textit{Rev.~Mod.~Phys.}~\textbf{74}, 1283} (2002)





















%\bibitem{stuhler} J. Stuhler, A. Griesmaier, T. Koch, M. Fattori, T. Pfau, S. Giovanazzi, P. Pedri, and L. Santos, Observation of Dipole-Dipole Interaction in a Degenerate Quantum Gas, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.95.150406}{\textit{Phys.~Rev.~Lett.}~\textbf{95}, 150406} (2005)

\bibitem{dynamic_alex1} A.~Filinov and M.~Bonitz, Collective and single-particle excitations in two-dimensional dipolar Bose gases, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.86.043628}{\textit{Phys.~Rev.~A} \textbf{86}, 043628} (2012)





%\bibitem{jan_willem} J.W.~Abraham and M.~Bonitz, Quantum Breathing Mode of Trapped Particles: From Nanoplasmas to Ultracold Gases, \href{https://onlinelibrary.wiley.com/doi/abs/10.1002/ctpp.201300066}{\textit{Contrib.~Plasma Phys.}~\textbf{54}, 27-99} (2014)






















% ### The UEG in general















%\bibitem{brualla} L.~Brualla, K.~Sakkos, J.~Boronat, and J.~Casulleras, Higher order and infinite Trotter-number extrapolationsin path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.1760512}{\textit{J.~Chem.~Phys.}~\textbf{121}, 636} (2004)

%\bibitem{sakkos} K.~Sakkos, J.~Casulleras, and J.~Boronat, High order Chin actions in path integral Monte Carlo, \href{https://aip.scitation.org/doi/abs/10.1063/1.3143522}{\textit{J.~Chem.~Phys.}~\textbf{130}, 204109} (2009)










%\bibitem{monte_carlo_book} G.~Fishman, Monte Carlo, \textit{Springer Series in Operations Research and Financial Engineering}, Springer, New York (1996)


























% benchmarking and guiding the development of new methods

\bibitem{panholzer1} M.~Panholzer, R.~Hobbiger, and H.~B\"ohm, Optimized correlations inspired by perturbation theory, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.99.195156}{\textit{Phys.~Rev.~B} \textbf{99}, 195156} (2019)




\bibitem{clark_casula} B.K.~Clark, M.~Casula, and D.M.~Ceperley, Hexatic and Mesoscopic Phases in a 2D Quantum Coulomb System, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.103.055701}{\textit{Phys.~Rev.~Lett.}~\textbf{103}, 055701} (2009)



%\bibitem{krauth_book} W.~Krauth,
%Statistical  Mechanics: Algorithms  and  Computations, \textit{Oxford Master Series in Physics}, Oxford University Press, 2006










\bibitem{dynamic_alex2} A.~Filinov, Correlation effects and collective excitations in bosonic bilayers: Role of quantum statistics, superfluidity, and the dimerization transition, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.94.013603}{\textit{Phys.~Rev.~A} \textbf{94}, 013603} (2016)











%\bibitem{greiner_book} W.~Greiner, D.~Rischke, L.~Neise, and H.~St\"ocker, Thermodynamics and Statistical Mechanics, Springer, New York (2012)


%\bibitem{janke} W.~Janke and T.~Sauer, Optimal energy estimation in path-integral Monte Carlo simulations, \href{https://aip.scitation.org/doi/abs/10.1063/1.474309}{\textit{J.~Chem.~Phys.}~\textbf{107}, 5821} (1997)






























% ### Here we introduce the frequency moments and stuff:

\bibitem{iwamoto2} N~Iwamoto, Inequalities for frequency-moment sum rules of electron liquids, \href{https://journals.aps.org/pra/abstract/10.1103/PhysRevA.33.1940}{\textit{Phys.~Rev.}~A \textbf{33}, 1940} (1985)


\bibitem{pines_woo} D.~Pines and C.-W. Woo, Sum Rules, Structure Factors, and Phonon Dispersion in Liquid $^4$He at Long Wavelengths and Low Temperatures, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.24.1044}{\textit{Phys.~Rev.~Lett.}~\textbf{24}, 1044} (1970)



\bibitem{kugler2} A.A.~Kugler, Bounds for Some Equilibrium Properties of an Electron Gas, \href{ http://link.aps.org/doi/10.1103/PhysRevA.1.1688}{ \textit{Phys.~Rev.~A} \textbf{1}, 1688} (1970)




\bibitem{puff1} R.D.~Puff, Application of Sum Rules to the Low-Temperature Interacting Boson System, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.137.A406}{\textit{Phys.~Rev.}~\textbf{137}, A406} (1965)

\bibitem{puff2} N.~Mihara and R.D.~Puff, Liquid Structure Factor of Ground-State He$^4$, \href{https://journals.aps.org/pr/abstract/10.1103/PhysRev.174.221}{\textit{Phys.~Rev.}~\textbf{174}, 221} (1968)




\bibitem{iwamoto} N.~Iwamoto, E.~Krotscheck, and D.~Pines, Theory of electron liquids. II. Static and dynamic form factors, correlation energy, and plasmon dispersion, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.29.3936}{\textit{Phys.~Rev.~B}~\textbf{29}, 3936} (1984)








\bibitem{dabrowski} B.~Dabrowski, Dynamical local-field factor in the response function of an electron gas, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.34.4989}{\textit{Phys.~Rev.~B}~\textbf{34}, 4989} (1986)








% Inserted by TD, to be sorted.


\bibitem{dornheim_FSC} T.~Dornheim and J.~Vorberger, Finite-size effects in the reconstruction of dynamic properties from ab initio path integral Monte-Carlo simulations, \href{https://arxiv.org/abs/2004.13429}{arxiv:2004.13429}


\bibitem{higuchi} M.~Highuchi and H.~Yasuhara, 
Kleinman's Dielectric Function and Interband Optical Absorption Strength of Simple Metals, \href{https://journals.jps.jp/doi/abs/10.1143/JPSJ.69.2099}{\textit{J.~Phys.~Soc.~Jpn.}~\textbf{69} 2099-2106} (2000)
 



\bibitem{Zastrau}
U. Zastrau, P. Sperling, M. Harmand, A. Becker, T. Bornath, R. Bredow, S. Dziarzhytski, T. Fennel,
L. B. Fletcher, E. Förster, S. Göde, G. Gregori, V. Hilbert, D. Hochhaus, B. Holst, T. Laarmann,
H. J. Lee, T. Ma, J. P. Mithen, R. Mitzner, C.D. Murphy, M. Nakatsutsumi, P. Neumayer, A. Przystawik,
S. Roling, M. Schulz, B. Siemer, S. Skruszewicz, J. Tiggesbäumker, S. Toleikis, T. Tschentscher,
T. White, M. Wöstmann, H. Zacharias, T. Döppner, S. H. Glenzer, and R. Redmer,
Resolving ultrafast heating of dense cryogenic hydrogen
\href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.112.105002}{\textit{Phys. Rev. Lett.}~\textbf{112}, 105002}  (2014)




\bibitem{benage} J.F.~Benage, W.R.~Shanahan, and M.S.~Murillo, Electrical Resistivity Measurements of Hot Dense Aluminum, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.83.2953}{\textit{Phys.~Rev.~Lett.}~\textbf{83}, 2953} (1999)


\bibitem{karasiev_importance} V.V.~Karasiev, L.~Calderin, and S.B.~Trickey, Importance of finite-temperature exchange correlation for warm dense matter calculations, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.93.063207}{\textit{Phys.~Rev.~E} \textbf{93}, 063207} (2016)



\bibitem{low_density1} S. Mazevet, M. P. Desjarlais, L. A. Collins, J. D. Kress, and N. H. Magee, Simulations of the optical properties of warm dense aluminum, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.71.016409}{\textit{Phys.~Rev.~E} \textbf{71}, 016409} (2005)

\bibitem{low_density2} M. P. Desjarlais, J. D. Kress, and L. A. Collins, Electrical conductivity for warm, dense aluminum plasmas and liquids, \href{https://journals.aps.org/pre/abstract/10.1103/PhysRevE.66.025401}{\textit{Phys.~Rev.~E} \textbf{66}, 025401(R)} (2002)

% References on dispersions
\bibitem{bohm-gross_49}
D. Bohm and E.P. Gross, 
Theory of Plasma Oscillations. A. Origin of Medium-Like Behavior,
Phys. Rev. \textbf{75}, 1851 (1949)

\bibitem{bohm-pines-3} D. Bohm, D. Pines, 
{A Collective Description of Electron Interactions: III. Coulomb
 Interactions in a Degenerate Electron Gas}, Phys. Rev. \textbf{92}, 609 (1952)

\bibitem{ferrell-57} R.A. Ferrell, 
{Characteristic Energy Loss of Electrons Passing through Metal Foils. II. Dispersion
Relation and Short Wavelength Cutoff for Plasma Oscillations},
Phys. Rev. \textbf{107}, 450 (1957)

\bibitem{thiele_pre_08} R. Thiele, T. Bornath, C. Fortmann, A. Höll, R. Redmer, H. Reinholz, G. Röpke, A. Wierling,
S. H. Glenzer, and G. Gregori,
Plasmon resonance in warm dense matter,
Phys. Rev. E \textbf{78}, 026411 (2008)

\bibitem{arista-brandt} N.R. Arista and W. Brandt, Dielectric response of quantum plasmas in thermal equilibrium, 
Phys. Rev. A \textbf{29}, 1471 (1984)

\bibitem{dandrea86} R.G. Dandrea, N. Ashcroft, and A.E. Carlsson, Electron liquid at any degeneracy, 
Phys. Rev. B \textbf{34}, 2097 (1986)

\bibitem{glenzer_rmp_09} S. Glenzer and R. Redmer, {X-ray Thomson scattering in high energy density plasmas},
Rev. of Mod. Phys. \textbf{81}, 1625 (2009)

\bibitem{bonitz_pop_94} M. Bonitz, Impossibility of Plasma Instabilities in Isotropic Quantum Plasmas, Phys. Plasmas \textbf{1}, 832 (1994)

\bibitem{bonitz_prl_93} M. Bonitz, R. Binder, and S.W. Koch, Carrier-Acoustic Plasmon Instability in Semiconductor Quantum Wires, Phys. Rev. Lett. \textbf{70}, 3788 (1993)

\bibitem{bonitz_pre_94} M. Bonitz, R. Binder, D.C. Scott, S.W. Koch,  and D. Kremp, Phys. Rev. E \textbf{49}, 5535 (1994)

\bibitem{vladimirov} S.V. Vladimirov and Y.O. Tyshetskiy, On description of a collisionless quantum plasma, Physics
Uspekhi \textbf{54}(12), 1243 (2011)


\bibitem{schakel} A.M.~Schakel, Ground state of electron gases at negative compressibility, \href{https://journals.aps.org/prb/abstract/10.1103/PhysRevB.64.245101}{\textit{Phys.~Rev.~B} \textbf{64}, 245101} (2001)

%%%%%%%%%%%
\end{thebibliography}

